PubSub-VFL: Towards Efficient Two-Party Split Learning in Heterogeneous Environments via Publisher/Subscriber Architecture

With the rapid advancement of the digital economy, data collaboration between organizations has become a well-established business model, driving the growth of various industries. However, privacy concerns make direct data sharing impractical. To address this, Two-Party Split Learning (a.k.a. Vertical Federated Learning (VFL)) has emerged as a promising solution for secure collaborative learning. Despite its advantages, this architecture still suffers from low computational resource utilization and training efficiency. Specifically, its synchronous dependency design increases training latency, while resource and data heterogeneity among participants further hinder efficient computation. To overcome these challenges, we propose PubSub-VFL, a novel VFL paradigm with a Publisher/Subscriber architecture optimized for two-party collaborative learning with high computational efficiency. PubSub-VFL leverages the decoupling capabilities of the Pub/Sub architecture and the data parallelism of the parameter server architecture to design a hierarchical asynchronous mechanism, reducing training latency and improving system efficiency. Additionally, to mitigate the training imbalance caused by resource and data heterogeneity, we formalize an optimization problem based on participants' system profiles, enabling the selection of optimal hyperparameters while preserving privacy. We conduct a theoretical analysis to demonstrate that PubSub-VFL achieves stable convergence and is compatible with security protocols such as differential privacy. Extensive case studies on five benchmark datasets further validate its effectiveness, showing that, compared to state-of-the-art baselines, PubSub-VFL not only accelerates training by $2 \sim 7\times$ without compromising accuracy, but also achieves a computational resource utilization rate of up to 91.07%.

==> sections/analysis.tex <==
\section{Convergence Analysis}


\subsection{Assumptions}
In this section, we provide the necessary assumptions as follows:

\begin{assumption}\label{ass-1}
(Smoothness). If the global loss function \(f(\theta)\) is \(L\)-smooth, thus, we have:
\begin{equation}
    \| \nabla f(\theta_1) - \nabla f(\theta_2) \| \le L \| \theta_1 - \theta_2 \|, \quad \forall \theta_1,\theta_2.
\end{equation}
\end{assumption}

\begin{assumption}\label{ass-2}
(Strong Convexity).  For the purpose of this analysis, we assume that \(f(\theta)\) is \(\mu\)-strongly convex:
\begin{equation}
f(\theta_2) \ge f(\theta_1) + \langle \nabla f(\theta_1), \theta_2 - \theta_1 \rangle + \frac{\mu}{2} \| \theta_2 - \theta_1 \|^2.    
\end{equation}
%For nonconvex losses, the analysis can be adapted to show convergence to a stationary point.
\end{assumption}

\begin{assumption}\label{ass-3}
(Bounded Stochastic Gradient Variance).  Let \(g(\theta; \xi)\) denote the stochastic gradient computed on a mini-batch. Then we have:
\begin{equation}
  \mathbb{E}\left[ \| g(\theta; \xi) - \nabla f(\theta) \|^2 \right] \le \sigma^2.  
\end{equation}
\end{assumption}

\begin{assumption}\label{ass-4}
(Bounded Delay/Staleness).  Due to semi‐asynchronous updates, the gradient used at iteration \(t\) is computed at a delayed parameter \(\theta_{t-\tau(t)}\) with \(\tau(t) \le \Delta T\). We assume that the delay satisfies
\begin{equation}
  \| \nabla f(\theta_t) - \nabla f(\theta_{t-\tau(t)}) \| \le L \sum_{j=t-\tau(t)}^{t-1} \| \theta_{j+1} - \theta_j \|.  
\end{equation}
\end{assumption}

\begin{assumption}\label{ass-5}
(Gaussian DP Noise Injection). The Gaussian noise \(\xi_{dp}\) added to each exchanged embedding is independent with
\begin{equation}
 \xi_{dp} \sim \mathcal{N}(0, \sigma_{dp}^2 I),   
\end{equation}
and the variance \(\sigma_{dp}^2\) is determined by the calibration formula provided. Consequently, the effective update noise is increased to
\begin{equation}
\sigma_{\text{total}}^2 = \sigma^2 + \sigma_{dp}^2.    
\end{equation}
\end{assumption}

\begin{assumption}\label{ass-6}
(Reliable Communication under Capacity Constraints). The Pub/Sub mechanism guarantees that embeddings (of dimension \(d\)) are delivered within the delay bound \(\tau\) provided that the channel capacity \(p\) is not exceeded.
\end{assumption}

\subsection{Convergence Analysis}
Based on the necessary assumptions above, we write the following convergence objective.

\begin{theorem}
If Assumptions \ref{ass-1}--\ref{ass-6} are held and if the update rule  
\begin{equation}
  \theta_{t+1} = \theta_t - \eta \Big( g_{t-\tau(t)} + \xi_{dp,t} \Big),  
\end{equation}
is applied with a constant learning rate \(\eta\) chosen sufficiently small (so that higher-order terms are negligible), there exist constants such that the expected optimality gap satisfies
\begin{equation}
\tiny
  \boxed{
\mathbb{E}\big[ f(\theta_t) - f(\theta^\ast) \big] \le \left(1 - 2\mu\eta + O\big(\eta^2 L + \eta^3 L^2 \tau\big)\right)^t \Big( f(\theta_0) - f(\theta^\ast) \Big) + \frac{L\eta \, (\sigma^2 + \sigma_{dp}^2)}{4\mu},
}  
\end{equation}
where \(\theta^\ast\) is the unique minimizer of \(f(\theta)\).
\end{theorem}
\begin{proof}
The detailed proof and deduction process are shown in the Appendix \ref{proof}.
\end{proof}

==> sections/background.tex <==
\section{Problem Formulation}
We consider a realistic scenario where two organizations collaboratively train an ML model to perform a prediction task (e.g., predicting a customer’s credit score). We then formalize a framework for VFL based on split learning, with the objective of maximizing the utilization of computing resources between two parties. In VFL, data is vertically partitioned such that each party holds different features for the same set of samples. Specifically, Active Party \( P_a \) possesses dataset \( D_1 = \{ (\mathbf{x}_i^a, y_i) \}_{i=1}^n \), where \( \mathbf{x}_i^a \in \mathbb{R}^{d_a} \) represents its feature vectors and \( y_i \in \mathbb{R} \) denotes the labels, while Passive Party \( P_p \) holds dataset \( D_2 = \{ \mathbf{x}_i^p \}_{i=1}^n \), with \( \mathbf{x}_i^p \in \mathbb{R}^{d_p} \). Note that the features of the two parties are disjoint. The model architecture is split into two parts: the top model and the bottom model, where the bottom models \( f_a(\cdot) \) and \( f_p(\cdot) \) are held by \( P_a \) and \( P_p \), respectively, while the top model \( g(\cdot,\cdot) \) is held by \( P_a \) which holds the label.

Before training begins, \( P_a \) and \( P_p \) must identify data samples with matching identifiers (such as ID). To preserve the privacy of both parties, Private Set Intersection (PSI)~\cite{chen2017fast} technique is typically employed to securely obtain the ``shared'' dataset without revealing any private information. During the forward pass, \( P_p \) computes an intermediate representation \( z_i^p = f_p(\mathbf{x}_i^p) \) (i.e., embeddings) and securely sends it to \( P_a \) by using methods like DP protocol, which then computes \( z_i^a = f_a(\mathbf{x}_i^a) \) and aggregates these representations using \( g(\cdot) \) to produce \( \hat{y}_i \), i.e., \( \hat{y}_i = g(f_a(\mathbf{x}_i^a), f_p(\mathbf{x}_i^p)) \). The loss function \( \mathcal{L}(\hat{y}_i, y_i) \) is calculated at \( P_a \). For example, for a classification task, the loss function can be the Cross-Entropy Loss:
\begin{equation}
\footnotesize
    \mathcal{L}(\hat{y}_i, y_i) = -\frac{1}{n} \sum_{i=1}^n \left( y_i \log(\hat{y}_i) + (1 - y_i) \log(1 - \hat{y}_i) \right).
\end{equation}
In the backward pass, \( P_a \) computes gradients \( \nabla_{z_i^a} \mathcal{L} \) and \( \nabla_{\theta_1} \mathcal{L} \), sending \( \nabla_{z_i^p} \mathcal{L} \) back to \( P_p \), which uses it to compute \( \nabla_{\theta_2} \mathcal{L} \). Both parties update their local model parameters using gradient descent:
\begin{equation}
{\theta _1} \leftarrow {\theta _1} - \eta {\nabla _{{\theta _1}}}\mathcal{L},{\theta _2} \leftarrow {\theta _2} - \eta {\nabla _{{\theta _2}}}\mathcal{L},
\end{equation}
where $\eta$ is the learning rate, and $\theta_1$ and $\theta_2$ are the network parameters of $f_1$ and $f_2$, respectively.

To maximize the utilization of computational resources, we need to balance the computational load between the two parties. Let \( Cost_A \) denote the computational cost of \( P_a \) for processing \(f_a\) and \( Cost_P \) denote the computational cost of \( P_p \) for processing \( f_p \). We use \( T_A \) to denote the total time taken by \( P_a \) for one iteration and use \( T_P \) to denote the total time taken by \( P_p \) for one iteration. The goal is to minimize the maximum time taken by either party, i.e., minimize \( \max(T_A, T_P) \). Assuming that the communication overhead is not negligible, we can write:
\begin{equation}
{T_A} = {Cost_A}+t_g ,{T_P} = {Cost_P}+t_e,
\end{equation}
where $t_g$ is time for sending gradient \( \nabla_{\theta_2} \mathcal{L} \) and $t_e$ is time for sending $z_i^p $. To balance the load, we aim to equalize \( T_A \) and \( T_P \): $ T_A \approx T_P$. This can be achieved by adjusting the training efficiency of \( f_a \) and \( f_p \) or dynamically allocating computing resources. For example, if \( Cost_A > Cost_P \), we can improve the training efficiency of \( f_a \) or increase the training efficiency of \( f_p \) to balance the workload. The formal objective is to minimize the maximum time taken by either party while ensuring convergence of the model:
\begin{equation}\label{eq-4}
     \min \max(T_A, T_P),
\end{equation}
subject to: $\frac{1}{n} \sum_{i=1}^n \mathcal{L}(\hat{y}_i, y_i) \leq \kappa$, where \( \kappa  \) is a small tolerance for the loss.

\para{Discussion.} Optimizing Eq. \eqref{eq-4} is a challenging task due to several key factors: 1) \textbf{Resource and Data Heterogeneity.} In practice, \( P_a \) and \( P_p \) often differ significantly in their computing resources and data dimensions. Additionally, \( P_p \)’s computational overhead in VFL is notably lower than \( P_a \)’s, as \( P_p \) does not need to perform a backward pass of the top model. Therefore, it is essential to balance resource allocation while accounting for the computational complexities of both parties. 2) \textbf{Privacy Restrictions.} Due to privacy concerns, it is not feasible to manage and control resource allocation in a centralized manner. This limitation distinguishes the problem from traditional resource scheduling in distributed learning, requiring more nuanced approaches to ensure privacy while optimizing resource utilization.

\para{Scarecrow Solution.} To optimize Eq. \eqref{eq-4}, a common approach is to implement a PS architecture within each party to achieve parallel processing. This architecture is widely adopted by industrial-level VFL frameworks like FATE~\cite{FATE2023} and PaddleFL~\cite{PaddleFL2023}. The PS architecture in VFL typically involves each party setting up a PS and a set of workers, each running a VFL executor responsible for model training and security protocols. For a given task, the coordinator, responsible for scheduling system components, determines the parallel factor \( \nu  \), which specifies the number of workers to be created. It then instructs the agents of each party to initiate the PS and workers. This setup involves both inter-party Peer-to-Peer communication among workers from different parties, as well as intra-party communication between the PS and its workers, ensuring efficient coordination and execution of the VFL task~\cite{wu2023falcon}.

Specifically, in each iteration, the $P_a$'s PS selects a batch and divides the instance IDs into \( q \) subsets, such as \( \text{ID} = \{ \text{ID}_1, \ldots, \text{ID}_q \} \). PS then broadcasts these subsets to the $P_p$'s PS, which distributes each subset \( \text{ID}_j \) to its workers. This ensures that during execution, the PS and workers of each party are aligned, with each group of workers processing the same instances. The workers of $P_a$ and $P_p$ execute forward propagation concurrently, with the workers of $P_a$ completing the remaining forward propagation and performing backward propagation using the top model. Meanwhile, once the workers of $P_p$ receive the corresponding gradients, they carry out backward propagation to update their local models. Afterward, each worker uploads the updated model parameters to its respective PS. Finally, the PS aggregates these updates and broadcasts the refined model parameters to its workers, completing the iteration.

\para{Limitations.} While deploying the PS architecture in VFL can significantly improve training efficiency (i.e., decrease \( Cost_1 \) and \( Cost_2 \)), it still faces certain limitations. Firstly, due to disparities in computational overhead among the parties, the computation times in VFL are unbalanced. Since PS must ensure strict ID alignment, the faster worker in a pair of workers must wait for the slower one, or the training process will fail due to mismatched embeddings. Moreover, deploying a PS does not fully address the issues of resource and data heterogeneity between parties, as the PS architecture cannot facilitate resource collaboration between different parties. This limits its ability to optimize resource allocation and manage data heterogeneity effectively in VFL.

==> sections/experment.tex <==
\section{Experiment}
\subsection{Experiment Setup}
To evaluate the performance of our \texttt{PubSub-VFL} system, we conduct extensive experiments on five datasets. All experiments are developed using Python 3.9 and PyTorch 1.12 and evaluated on a server with an INTEL(R) XEON(R) GOLD 6530 (64-core CPU).

\para{Datasets.} We evaluate \texttt{PubSub-VFL} on four public benchmark datasets covering both regression and classification tasks, as well as a synthetic large-scale dataset. Specifically, for regression tasks, we use the Energy~\cite{appliances_energy_prediction} dataset (19,735 samples, 27 features) and the Blog~\cite{blog_feedback} dataset (60,021 samples, 280 features). For classification tasks, we use the Bank~\cite{bank_marketing} dataset (40,787 samples, 48 features) and the Credit~\cite{credit_card_default} dataset (30,000 samples, 23 features). To assess scalability, we generate a synthetic dataset with 100,000 samples and 500 features using the Sklearn toolkit~\cite{scikit-learn}. The datasets cover different objects, domains, attributes, dimensions, and number of classes, as shown in Table \ref{tab:dataset_summary}, allowing us to explore the learning effectiveness of \texttt{PubSub-VFL}. We split each dataset into training and test sets in a 7:3 ratio, distributing the training data approximately evenly between the two parties. Note that in all experiments, only the $P_a$ holds the labels. To simulate data heterogeneity, we vary the number of features allocated to different parties (see details below).


\para{Models.} For the top model, we use a Multi-Layer Perceptron (MLP) with two layers. For the bottom model, we use two models of different sizes, namely a ten-layer MLP (small-size model) and a ResNet~\cite{he2016deep} (large-size model), which can verify the performance of PubSubVFL under different model sizes.


\para{Parameters.} For a series of constants, we set $\Delta T_0=5$, $T_{ddl}=10s$, $p=5$, $q=5$. For the constants in the optimization model, we determined them through empirical experiments (see the Appendix \ref{exper} for details). In addition, we set the learning rate to 0.001, the number of workers to $w_a/w_p \in [2,50]$, the batch size $B\in\{16,32,64,128,256,512,1024\}$, and $C_a+C_p=64$.

\para{Baselines.} In this paper, we adopt the following baselines:

\textit{Pure VFL.} This is a classic VFL architecture that does not involve the PS architecture or asynchronous mechanisms.

\textit{VFL with PS.} This is the most widely adopted VFL architecture in the industry, implemented in mature frameworks such as FATE~\cite{FATE2023} and PaddleFL~\cite{PaddleFL2023}. By leveraging the PS architecture, it enhances computational resource utilization and efficiency, enabling more effective parallel processing.

\textit{Asynchronous VFL.} Building on traditional VFL, developers can integrate asynchronous mechanisms~\cite{zhang2024asynchronous,zhang2021secure} to implement Asynchronous VFL (AVFL), enhancing system efficiency by reducing idle time and improving parallelism.

\textit{Asynchronous VFL with PS.} Building on AVFL, developers can integrate the PS mechanism~\cite{wu2023falcon} to further enhance VFL efficiency. Notably, the asynchronous implementation in this architecture is achieved through inter-party communication between parties.

We emphasize that certain algorithms that are well suited for VFL, e.g., asynchronous SGD~\cite{zhang2021asysqn, chen2017fast}, are not used as baselines because they are not applicable to SL-based VFL.

%Additionally, we highlight that certain algorithms, such as asynchronous SGD~\cite{zhang2021asysqn,chen2017fast} and gradient compression~\cite{castiglia2022compressed}, which are well-suited for VFL, are not applicable to the SL-based VFL architecture studied in this paper. This limitation arises because the intermediate interaction results in SL-based VFL involve both embeddings and gradients.

\para{Evaluation Metrics.} For the four public benchmark datasets, we evaluate classification tasks using the Area Under the ROC Curve (AUC) and regression tasks using the Root Mean Square Error (RMSE). For the synthetic dataset, we use AUC as the evaluation metric for classification tasks. To fairly assess computational resource utilization, we measure running time, CPU utilization, and waiting time/epoch. Additionally, we record communication cost to compare the communication efficiency of different methods.
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}[!t]
\caption{Accuracy comparison on benchmark datasets.}
\vspace{-0.4cm}
\label{tab-1}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{llccccc}
\toprule
\textbf{Dataset}                   & \textbf{Metric}   & \textbf{VFL} & \textbf{VFL-PS} & \textbf{AVFL} & \textbf{AVFL-PS} & \textbf{Ours} \\ \hline
{Energy}    & \textbf{RMSE}      &84.58     &84.44        &85.41      &85.39         &{85.64}      \\
                   
{Blog}      & \textbf{RMSE}      &23.20     &23.12        &23.38      &23.45         &\textbf{22.34}      \\
 
                 
{Bank}      & \textbf{AUC}      &94.54     &94.13        &94.12      &94.16         &\textbf{96.54}      \\
                  
{Credit}    & \textbf{AUC}      &81.90     &81.34        &80.83      &80.34         &  \textbf{82.34}       \\
                   
{Synthetic} & \textbf{AUC}      & 91.27   & 91.31       & 90.97     & 91.21        &   \textbf{92.87}   
                               \\ \bottomrule
\end{tabular}%
}
\vspace{-0.5cm}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!t]
\caption{Effect of the number of workers.}
\vspace{-0.4cm}
\label{tab-2}
\resizebox{0.45\textwidth}{!}{%
\begin{tabular}{lccccccc}
\toprule
\# of Workers          & 4      & 5       & \textbf{8*}     & 10      & 20      & 30      & 50      \\ \hline
Acc.(\%)             & 92.13  & 92.05   & \textbf{92.06}  & 92.28   & 92.00   & 92.36   & 92.21   \\
Running Time (s)     & 712.78 & 805.90  & \textbf{668.11} & 885.01  & 1420.32 & 1067.57 & 1661.74 \\
CPU Utilization (\%) & 67.52  & 63.30   & \textbf{88.04}  & 76.18   & 42.77   & 40.78   & 45.12   \\
Waiting Time (s)    & 1.4686 & 1.9273  & \textbf{1.5288} & 3.461   & 8.088   & 9.687   & 19.843  \\
Comm. Overhead (MB)  & 878.91 & 1098.63 & \textbf{888.77} & 1318.36 & 1867.68 & 1538.09 & 2197.27 \\ \hline
\end{tabular}%
}
\vspace{-0.45cm}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!t]
\caption{Effect of the different batch size.}
\vspace{-0.4cm}
\label{tab-3}
\resizebox{0.45\textwidth}{!}{% 从 0.45 增大到 0.5
\begin{tabular}{lccccccc}
\toprule
Batch Size           & 16     & 32      & 64     & {128}    & \textbf{256}     & 512     & 1024    \\ \hline
Acc.(\%)             & 91.70   & 92.06  & 91.75  & 92.63  & \textbf{92.67}  & 92.36  & 92.21   \\
Running Time (s)     & 987.64  & 668.11 & 344.76 & 124.01 & \textbf{92.54}  & 578.69 & 865.74  \\
CPU Utilization (\%) & 48.64   & 88.04  & 90.12  & 89.97  & \textbf{91.07}  & 84.47  & 52.67   \\
Waiting Time (s)    & 1.087   & 1.5288 & 1.688  & 1.263  & \textbf{1.1389} & 1.324  & 1.789   \\
Comm. Overhead (MB)  & 1298.32 & 888.77 & 329.59 & 439.45 & \textbf{439.45} & 736.89 & 1070.36 \\ \hline
\end{tabular}%
}
\vspace{-0.5cm}
\end{table}
\subsection{Numerical Results}


\para{System Performance.} We evaluate the performance of \texttt{PubSub-VFL} and baseline methods on five datasets across classification and regression tasks. To ensure a balanced allocation of resources and data, we evenly distribute CPU cores and feature sizes between the two parties. Additionally, to assess the impact of different bottom model architectures, we employ both MLP and ResNet models. We report the best performance of each method under optimal hyperparameter configurations in Tables \ref{tab-1} and \ref{tab:my-table-2}. The experimental results demonstrate that \texttt{PubSub-VFL} achieves accuracy comparable to or even surpassing baseline methods on the Bank, Credit, and Synthetic datasets. This confirms that integrating the Pub/Sub architecture and semi-asynchronous mechanism does not compromise system performance or convergence.







\begin{figure*}[!t]
\centering
    \subfigure{
    \includegraphics[width=0.8\linewidth]{figs/fig-legend.pdf}
    }
    \vspace{-15pt}
    \\
    \addtocounter{subfigure}{-1}
   \subfigure[Running Time]{
   \includegraphics[width=0.235\linewidth]{figs/fig-8-1.pdf}
   }
  \subfigure[CPU Utilization]{
  \includegraphics[width=0.235\linewidth]{figs/fig-8-2.pdf}
  }
   \subfigure[Waiting Time]{
   \includegraphics[width=0.235\linewidth]{figs/fig-8-3.pdf}
   }
      \subfigure[Comm. Cost]{
   \includegraphics[width=0.235\linewidth]{figs/fig-8-4.pdf}
   }
   \vspace{-0.5cm}
  \caption{Comparison with existing baselines in computation and communication efficiency.} \label{fig-3}
\vspace{-0.5cm}
\end{figure*}

\begin{figure*}[!t]
\centering
    \subfigure{
    \includegraphics[width=0.8\linewidth]{figs/fig-legend.pdf}
    }
    \vspace{-15pt}
    \\
    \addtocounter{subfigure}{-1}
   \subfigure[Running Time]{
   \includegraphics[width=0.235\linewidth]{figs/fig-10-1.pdf}
   }
  \subfigure[CPU Utilization]{
  \includegraphics[width=0.235\linewidth]{figs/fig-10-2.pdf}
  }
   \subfigure[Running Time]{
   \includegraphics[width=0.235\linewidth]{figs/fig-10-3.pdf}
   }
      \subfigure[CPU Utilization]{
   \includegraphics[width=0.235\linewidth]{figs/fig-10-4.pdf}
   }  
   \vspace{-0.5cm}
  \caption{Comparison with existing baselines on computation efficiency in resource and data heterogeneous scenarios.} \label{fig-4}
\vspace{-0.5cm}
\end{figure*}
\begin{figure*}[!t]
\centering
    \subfigure{
    \includegraphics[width=0.6\linewidth]{figs/fig-line-legend.pdf}
    }
    \vspace{-15pt}
    \\
    \addtocounter{subfigure}{-1}
   \subfigure[Accuracy]{
   \includegraphics[width=0.235\linewidth]{figs/fig-7-1.pdf}
   }
  \subfigure[CPU Utilization]{
  \includegraphics[width=0.235\linewidth]{figs/fig-7-2.pdf}
  }
   \subfigure[Comm. Cost]{
   \includegraphics[width=0.235\linewidth]{figs/fig-7-3.pdf}
   }
      \subfigure[ASR]{
   \includegraphics[width=0.235\linewidth]{figs/fig-7-4.pdf}
   }  
   \vspace{-0.5cm}
  \caption{The impact of privacy budget on the performance, efficiency, and security of \texttt{PubSub-VFL.}} \label{fig-5}
\vspace{-0.5cm}
\end{figure*}
\para{Computational \& Communication Efficiency.} We evaluate the computational and communication efficiency of \texttt{PubSub-VFL} compared to baseline methods. We apply our proposed optimization method to determine the best hyperparameters (i.e., $B=256, w_a=8, w_p=10$) for configuring \texttt{PubSub-VFL}. For computational efficiency, we measure the running time, CPU utilization, and waiting time/epoch required to reach a specified accuracy (i.e., 91\%). For communication efficiency, we assess the communication cost of different methods. Extensive evaluations on the synthetic dataset demonstrate that \texttt{PubSub-VFL} significantly outperforms baseline methods in computational efficiency and resource utilization. Specifically, in Fig. \ref{fig-3}, \texttt{PubSub-VFL} achieves a $7\times$ reduction in running time and 35\% higher CPU utilization compared to the best baseline (i.e., AVFL-PS), thanks to its ability to minimize worker idle time and enhance parallel processing efficiency. \texttt{PubSub-VFL} also reduces communication cost relative to other baselines, as its hierarchical asynchronous mechanism improves convergence efficiency.

\para{Resource and Data Heterogeneity Scenarios.} We evaluate the computational efficiency of \texttt{PubSub-VFL} and the baseline methods under varying resource allocation and feature size distribution scenarios. For the resource heterogeneous scenario, we set different CPU core ratios between $P_a$ and $P_p$: 50:14, 48:16, 40:24, and 36:28 (where the first value represents $P_a$'s CPU cores). For the data heterogeneous scenario, we set different feature size ratios: 50:450, 100:400, 150:350, and 200:300. In each scenario, we apply our optimization method to determine the best hyperparameters and configure them for \texttt{PubSub-VFL}. The experimental results, shown in Fig. \ref{fig-4}, reveal that in the resource heterogeneous scenario, imbalanced computational efficiency between parties significantly increases waiting time and decreases CPU utilization in baseline methods. Specifically, the CPU utilization of \texttt{PubSub-VFL} is still as high as 87.42\% when the CPU core ratio is 50:14, while that of AVFL-PS is only 42.12\%. This happens because resource disparities exacerbate computational imbalances, further extending training latency. In contrast, \texttt{PubSub-VFL} effectively balances computational efficiency, reducing running time and maintaining high CPU utilization. In the data heterogeneity scenario, we observe similar trends. Additionally, we find that reducing the data dimension processed by $P_a$ can further decrease running time (as shown in Fig. \ref{fig-4} (c)--(d)). This is because it helps balance the computational load between both parties, aligning with our optimization model design approach.





\para{Security Performance Evaluation.} We evaluate it from two dimensions: system performance and defense against embedded inversion attacks~\cite{song2020information}. We follow the above hyperparameter configuration to configure \texttt{PubSub-VFL}. For the privacy parameter, we set $\mu \in \{0.1, 0.5, 1, 2, 4, 8, 10, + \infty \}$. %More experimental results can be found in the Appendix.

\textit{System Performance.} We evaluate the impact of $\mu$ on \texttt{PubSub-VFL} by recording its accuracy, CPU utilization, and communication cost on the Bank, Credit, and Synthetic datasets. The results, presented in Fig. \ref{fig-5}, demonstrate that introducing the DP protocol has minimal effect on accuracy and CPU utilization, indicating that \texttt{PubSub-VFL} maintains its computational efficiency even with privacy protection. However, we observe a notable increase in communication cost due to the added DP noise, which leads to a slower convergence. Nevertheless, the results confirm that \texttt{PubSub-VFL} seamlessly integrates with security protocols while maintaining strong performance. %Results on other datasets can be found in the Appendix \ref{exper}.


\textit{Defend Against Embedding Inversion Attacks (EIA).} Similarly, we record the performance results (i.e., Attack Success Rate (ASR)) of \texttt{PubSub-VFL} against EIA (we adopt it in \cite{song2020information}) on these datasets (more details can be found in the Appendix \ref{EIA}). The results are shown in Fig. \ref{fig-5}, showing that the introduction of the DP protocol can help \texttt{PubSub-VFL} defend against EIA well.



\para{Parameter Sensitivity Evaluation.} We evaluate the impact of different numbers of workers and batch sizes on the performance of \texttt{PubSub-VFL} under the same setting. Specifically, we set $w_a=w_p \in \{4, 5, 8, 10, 20, 30, 50\}$ and $B \in \{16, 32, 64, 128, 256, 512, 1024\}$.

\textit{Effect of the Numer of Workers.} We conduct experiments on the Synthetic dataset with $B=32$, and the experimental results are shown in Table \ref{tab-2}. The results show that simply increasing the parallel factor (i.e., $w$) does not always improve computational efficiency. For example, we find that when $w = 8$, its computation and communication efficiency is the highest. This is because a large parallel factor will lead to slower convergence.


\textit{Effect of the Batch Size.} Similarly, we conduct experimens on the Synthetic dataset with $w_a=w_p=8$. Table \ref{tab-3} records the impact of different $B$ on the performance of \texttt{PubSub-VFL}. We find that blindly increasing $B$ cannot always improve the computational efficiency of \texttt{PubSub-VFL}. For example, we find that when $B = 256$, its computation and communication efficiency is the highest. This is because too large a batch size will also lead to slower convergence. The above results verify that we need a suitable method to find the optimal hyperparameters in the VFL task.



%\para{Ablation Studies (RQ6).} 




\section{Conclusion}
The paper addressed the problem of underutilization of computational resources in VFL by proposing a new framework named \textsf{PubSub-VFL}. Specifically,  \texttt{PubSub-VFL} enhanced computational efficiency by leveraging a Pub/Sub architecture with hierarchical asynchronous mechanism. Furthermore, we theoretically prove the convergence of \textsf{PubSub-VFL}. It reduces training latency, improves resource utilization, and maintains strong convergence and privacy guarantees, achieving up to $2\sim7\times$ faster training and $ \approx 35\%$ better resource efficiency than state-of-the-art baselines.

==> sections/intro.tex <==
\section{Introduction}
In the digital economy, data has become a crucial resource driving technological advancements in sectors like autonomous driving~\cite{zheng2023autofed}, healthcare~\cite{ogier2022flamby}, and e-commerce~\cite{li2024federated}. In this context, enterprises are increasingly collaborating to aggregate diverse data sources to train Machine Learning (ML) models, improving user experience and efficiency~\cite{zhang2020batchcrypt}. However, centralized data collection poses significant privacy risks and potential breaches~\cite{liu2022privacy}. Additionally, regulations like the General Data Protection Regulation (GDPR)~\cite{voigt2017eu} impose strict limits on data aggregation and usage, requiring explicit consent and robust safeguards.

To address the above privacy concerns, enterprises generally deploy Vertical Federated Learning~\cite{liu2024vertical,yang2019federated,wang2024unified,qi2022fairvfl} to collaboratively train ML models without accessing the original data. Specifically, in VFL, the data is partitioned vertically, such that each party stores data corresponding to the same sample IDs but with different feature spaces~\cite{wang2024unified,huang2023vertical,xing2024preventing}. This allows for a comprehensive analysis through a secure exchange of intermediate results, protecting sensitive data while facilitating joint model training~\cite{liu2024vertical,jin2021cafe}. A notable example is the cooperation between banks and insurance companies aiming to train a model to predict a customer's credit score, a common interest for both entities. Each party holds data on the same individuals but in different feature spaces: banks maintain financial transaction records, while insurance companies retain car accident reports. Due to privacy concerns, regulatory constraints (such as GDPR and HIPAA~\cite{gostin2009beyond}), and communication network limitations, these features must remain localized within each party. In such scenarios, the VFL approach becomes essential. Therefore, many efforts~\cite{zhang2021asysqn,ogier2022flamby,gu2020federated} have been invested in VFL research to further unlock the commercial value of data.

In the above scenarios, split-learning-based VFL~\cite{fu2022blindfl,thapa2022splitfed} is frequently employed, as shown in Fig. \ref{fig-1}. In this framework, each party trains a partial deep network up to a specific layer known as the cut layer (called \emph{bottom model}), which maps raw data features into meaningful vector representations or \emph{embeddings} for prediction tasks. These embeddings are securely transmitted (using methods like differential privacy~\cite{dwork2006differential}, homomorphic encryption~\cite{zhang2020batchcrypt}, or secure multi-party computation~\cite{ogier2022flamby}) to the \emph{active party}, which holds the labeled data. The active party completes the training using the remaining part of the network (called \emph{top model}) without accessing the raw data of the other parties, thus completing a forward propagation round. Subsequently, gradients are back-propagated from the final layer of the top model to the cut layer. Only the gradients at the cut layer are sent back to the \emph{passive parties}, who then continue the backpropagation process locally. This iterative process is repeated until the model converges. However, in practice, this architecture often suffers from low training efficiency and low resource utilization due to synchronization dependencies~\cite{zhang2021asysqn,castiglia2023less,castiglia2022compressed,wang2024unified}.


In light of these challenges, researchers and developers are dedicated to designing efficient VFL architectures to enhance computational resource utilization and improve training efficiency. From a system-level perspective, previous works such as FATE~\cite{FATE2023} and PaddleFL~\cite{PaddleFL2023} have focused on achieving efficient data parallelism by employing Parameter Server (PS)~\cite{li2014scaling} architectures, thereby significantly improving computational resource utilization. At the algorithmic level, considerable effort has been devoted to developing effective asynchronous VFL training protocols, such as Asynchronous Stochastic Gradient Descent (AsySGD~\cite{gu2020unified,zhang2024asynchronous}), and fast-convergence algorithms like AsySQN~\cite{zhang2021asysqn}, to optimize computational efficiency. However, these methods still face limitations. Some approaches may not fully address computational bottlenecks, while others might fail to maximize computational efficiency under resource and data heterogeneity conditions. We highlight the reasons behind the above design deficiencies as follows:

\begin{icompact}
\item \textbf{Ignoring the Decoupling of the System.} Since the VFL with PS setup is still synchronous and tightly coupled, there is a waiting bottleneck between workers on different parties~\cite{wu2023falcon}, where they either wait for each other or have computational dependencies (see Fig. \ref{fig-12}). Introducing an asynchronous mechanism could potentially improve system decoupling. However, the unique characteristics of the VFL ID alignment~\cite{he2022differentially} present significant challenges in implementing such a mechanism directly (see the detailed analysis below).
\item \textbf{Ignoring Resource and Data Heterogeneity.} In VFL, computational resource and data feature dimensions often vary significantly among parties, leading to imbalances in computing time~\cite{castiglia2022compressed,li2024convergence}. Existing methods typically focus on incrementally improving the computational efficiency of individual parties, overlooking these discrepancies. Thus, the overall computational resources are underutilized due to the lack of a holistic approach to addressing this issue.
\end{icompact}
\begin{figure}[!t]
    \centering
    \includegraphics[width=0.30\textwidth]{figs/fig-5.pdf}
    \vspace{-0.4cm}
    \caption{Overview of the SL-based VFL framework.}
    \label{fig-1}
    \vspace{-0.5cm}
\end{figure}

To address the limitations of existing approaches, we propose an efficient VFL framework named \texttt{PubSub-VFL}, designed to achieve better computational resource utilization and improve training efficiency. \texttt{PubSub-VFL} combines the loose coupling advantages of the Publisher/Subscriber (Pub/Sub) architecture with the data parallelism benefits of the PS architecture, enabling flexible asynchronous communication and significantly enhancing system throughput. To further boost computational efficiency and ensure convergence, we design an adaptive semi-asynchronous mechanism within the PS, forming a hierarchical asynchronous mechanism in conjunction with the Pub/Sub asynchrony outside the PS. Additionally, to tackle load imbalance issues caused by resource and data heterogeneity, we develop an optimization model that leverages system profile information to determine optimal hyperparameters, thereby further improving resource utilization. Extensive evaluations on five benchmark datasets demonstrate that \texttt{PubSub-VFL} achieves a $2\sim 7\times$ improvement in computational efficiency over state-of-the-art baselines while maintaining model accuracy. Our contributions can be summarized as follows:
\begin{icompact}
     \item We design \texttt{PubSub-VFL}, an advanced VFL framework designed for efficient computational resource utilization in two-party collaborative learning. 
    \item We propose a convergent hierarchical asynchronous mechanism that minimizes idle time while ensuring stable model convergence. Additionally, we formalize an optimization problem that determines the best hyperparameter configuration for \texttt{PubSub-VFL} in a privacy-preserving manner.
    \item Extensive experiments on five datasets demonstrate the superior performance of \texttt{PubSub-VFL}. Specifically, it achieves $2 \sim 7\times$ faster training speeds and 91.07\% resource utilization, surpassing advanced baselines, all without compromising model accuracy.  
\end{icompact}

%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=0.4\textwidth]{figs/fig-11.pdf}
%    \vspace{-0.4cm}
%    \caption{(Left) Due to synchronization dependency, limited computational resources on party B can cause party A to experience extended waiting times. (Middle) If party B encounters a failure or delay, party A is forced to wait, leading to increased training latency. (Right) Even if an asynchronous mechanism is used, due to the need for ID alignment, if party A calculates too fast or too slow, it will cause a mismatch with the batch required by party B.}
%    \label{fig-11}
%    \vspace{-0.5cm}
%\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=0.35\textwidth]{figs/fig-12.pdf}
    \vspace{-0.4cm}
    \caption{Pipeline overview of the VFL with PS architecture. Synchronization dependencies may cause latency 1 and latency 3, while latency 2 is the computation dependency caused by ID alignment.}
    \label{fig-12}
    \vspace{-0.5cm}
\end{figure}


==> sections/method.tex <==
\begin{figure*}[!t]
 \centering
 \includegraphics[width=13cm, height=4cm]{figs/fig-6.pdf} % 修改为固定宽度和高度
 \vspace{-0.4cm}
 \caption{System architecture and workflow of \texttt{PubSub-VFL}.}
 \label{fig-2}
 \vspace{-0.5cm}
\end{figure*}
\section{System and Algorithm Design}
%In this section, we present the designed \texttt{PubSub-VFL} system, which involves three stages: system design, system profiling, and algorithm design. Next, we will introduce each stage in detail.

\para{Overview.} Fig. \ref{fig-2} illustrates the workflow and system architecture of \texttt{PubSub-VFL}, which features three primary phases: profiling, planning, and execution. We first elaborate on the system design of \texttt{PubSub-VFL}, which integrates the Pub/Sub architecture, PS architecture, and key components like the hierarchical asynchronous mechanism, buffer mechanism, and waiting deadline mechanism to improve training efficiency (see \S\ref{4-2}). In the profiling phase, the system uses a calibration dataset to collect runtime profiles, which are essential for efficient parallel planning (see \S\ref{4-3}). During the planning phase, these profiles inform the generation of hyperparameter configurations, including the number of workers and batch allocation, to address the resource and data heterogeneity challenges (see \S\ref{4-4}). Finally, in the execution phase, the task publisher uses the system to carry out model execution, exchange intermediate results, and aggregate updates. %This structured process ensures optimal resource utilization and system performance throughout the collaborative learning task.

%\para{Core Challenge.} Given the above limitations, our primary objective is to eliminate the waiting delays between corresponding workers, thereby enhancing training efficiency. The core challenge lies in \emph{eliminating these delays without compromising data ID alignment}. A natural solution is to introduce an asynchronous mechanism to mitigate worker delays. However, while asynchrony can reduce waiting times by allowing workers to continue with other tasks during delays, it does not ensure that corresponding workers will maintain data ID alignment in each iteration. This misalignment occurs because the asynchronous mechanism permits independent progression of tasks, potentially leading to inconsistencies in data processing across workers. Thus, addressing this challenge requires a more nuanced approach to maintain alignment while leveraging the benefits of asynchrony.

\subsection{System Design}\label{4-2}

\para{Key Idea.} To address the scarecrow solution's limitations, our key idea is to \emph{decouple the data ID alignment task from the training tasks of workers across different parties.} This approach allows workers to focus solely on local training without the need to ensure data ID alignment beforehand. To implement this, we introduce the \emph{Publisher/Subscriber} (Pub/Sub)~\cite{srivatsa2011eventguard} architecture, which effectively separates the training process from the data ID matching task, enabling asynchronous operations while maintaining the necessary alignment. By doing so, we can eliminate waiting delays, improve system concurrency, and ensure seamless data ID alignment without burdening the workers with additional coordination tasks. More information about the Pub/Sub can be found in the Appendix~\ref{pubsub}.

To this end, we present the designed \texttt{PubSub-VFL} system as follows. Specifically, as shown in Fig. \ref{fig-2}, we designate channels or topics to facilitate seamless integration into VFL by establishing \emph{gradient channels} and \emph{embedding channels}. The gradient channels handle the exchange of gradients between the parties, while the embedding channels manage the transfer of embeddings. To decouple the training task from the data ID alignment task, we predefine a unique batch ID for each training data batch and assign this identifier to the corresponding communication channel. Each channel, whether for gradients or embeddings, is uniquely identified by its batch ID. With this setup, workers can send their intermediate computation results to the appropriate channel based on the matching batch ID, eliminating the need to wait for other workers. Assuming the total number of data IDs is \( \lceil n/B \rceil \), where \( B \) is the batch size, the number of gradient channels or embedding channels will also be \( \lceil n/B \rceil \). By this way, the proposed system ensures that each batch's data remains properly aligned across parties, while allowing workers to operate asynchronously, improving overall training efficiency. 

In a more practical scenario, computationally efficient workers may generate excessive embeddings or gradients, leading to channel congestion, which can impede model convergence or even cause training failures. To address this, we propose two mechanisms:
\begin{icompact}
\item  \textbf{Buffer Mechanism:} Each channel buffer can store up to \( p \) embeddings and \( q \) gradients, with each entry timestamped. When the buffer reaches its capacity, it discards the oldest embedding or gradient based on a First-In-First-Out (FIFO)~\cite{herr2003implementation} principle to prevent stale updates from affecting the training process.
\item \textbf{Waiting Deadline Mechanism:} If a subscribing worker does not receive the embedding or gradient from the publishing worker within a predetermined time \( T_{ddl} \), it discards the current batch and notifies the other party to proceed with the next batch. The system then reassigns the batch to any available pair of workers for retraining, ensuring the continuity of the training process and mitigating delays caused by congestion. 

\end{icompact}
%These mechanisms help maintain smooth data flow and ensure robust model training despite potential bottlenecks.

\para{Intra-party Semi-asynchronous Mechanism.} From the above Pub/Sub architecture design, it is evident that we have achieved inter-party asynchronous communication, effectively eliminating the waiting delays for workers. To further enhance computational efficiency within each party, i.e., between the PS and workers, we also implement an asynchronous mechanism. However, this hierarchical asynchronous approach may complicate or hinder model convergence. To address this challenge, we propose a dynamic semi-asynchronous mechanism within each party to accelerate convergence. This mechanism dynamically adjusts the level of asynchrony based on real-time feedback from the training process, balancing the need for faster computations with the stability required for model convergence. To implement a dynamic semi-asynchronous mechanism in a PS architecture for VFL, the synchronization interval \( \Delta T_t \) is designed to decrease as the model approaches the target accuracy. The interval \( \Delta T_t \) is defined as:
\begin{equation}
\Delta {T_t} = \left\lceil {\frac{{\Delta {T_0}}}{2} \cdot \tanh \left( {\frac{{2 \cdot t}}{{\Delta {T_0}}} - 2} \right) + \frac{{\Delta {T_0}}}{2}} \right\rceil,
\end{equation}
where $\Delta T_0$ is the initial asynchronous interval, $t$ is the current training epoch, and ${\tanh ( \cdot )}$ is the hyperbolic tangent function. Initially, when the model is far from the target accuracy, \( \Delta T_t \) is small, allowing the model to achieve stable learning. As the accuracy increases, the interval increases and the synchronization frequency is reduced to fine-tune the model and ensure faster convergence. %This approach balances computational efficiency with convergence speed, adapting dynamically to the model's progress.


\para{Differential Privacy Protocol.} To prevent the embedded information sent by \( P_p \) from being inferred by attackers (such as labels or features), specific perturbations must be added to the embeddings. To balance privacy and utility effectively, we adopt Gaussian Differential Privacy (GDP) as outlined in \cite{dwork2006differential,chen2020vafl} to safeguard the embedding information. The formal definition of GDP is as follows:
\begin{definition}
\label{def:inj}
A randomized mechanism \( \mathcal{M} \) satisfies \( (\mu, \sigma_{dp}) \)-GDP if for all measurable sets \( S \) and for all adjacent datasets \( D \) and \( D' \), the following inequality holds:
\begin{equation}\label{eq-6}
\mathbb{P}[\mathcal{M}(D) \in S] \leq e^{\mu} \mathbb{P}[\mathcal{M}(D') \in S] + \delta,
\end{equation}
where \( \mu \) is a privacy loss parameter, \( \sigma_{dp} \) is the standard deviation of the Gaussian noise added, and \( \delta \) is a small probability allowing for a slight relaxation of the privacy guarantee. We explain the GDP design applicable to the embedding mechanism in the Appendix~\ref{dp}.
\end{definition}


\subsection{System Profiling Phase}\label{4-3}
\para{Key Idea.} \texttt{PubSub-VFL} effectively leverages the Pub/Sub and PS architectures to unleash the computing power of parties, significantly enhancing training efficiency. However, this system still struggles to mitigate computing latency issues arising from resource and data heterogeneity. The core challenge lies in the difficulty of collaboratively allocating resources without compromising privacy. To tackle this, our key approach is to determine a set of optimal parameters, such as the number of workers, batch size, and allocation of computing cores, based on the system profiles of both parties, which include model information and hardware capabilities. By tailoring these parameters to the specific resources and constraints of each participant, we aim to balance the computational load, reduce latency, and enhance the overall efficiency of the VFL system, all while maintaining privacy compliance.

To achieve this goal, we first model the computation and communication delays of both the active and passive parties in the designed \texttt{PubSub-VFL} system. For the $P_a$, we denote the number of workers as \( w_a \in [P, Q] \), batch size as \( B \), and total computing cores as \( C_a \). For the $P_p$, the number of workers is \( w_p \in [M, N] \), batch size as \( B \), and total computing cores as \( C_p \). Let \(\{c_{a,i}\}_{i=1}^{w_a}\) (where \(\sum_{i=1}^{w_a} c_{a,i} \; \le \; C_a\), be the CPU cores allocated to each of the \(w_a\) and \(\{c_{p,j}\}_{j=1}^{w_p}\) (where \(\sum_{j=1}^{w_p} c_{p,j} \; \le \; C_p\)) be the CPU cores allocated to each of the \(w_p\). Therefore, the computation delay of the forward pass of both parties can be formally defined as follows:
\begin{equation}\label{eq-7}
T_f^{(a)}(B) = \frac{{{\lambda _a}{B^{{\gamma _a}}}}}{{\sum\limits_{j = 1}^{{w_a}} {{c_{a,j}}} }},T_f^{(p)}(B) = \frac{{{\lambda _p}{B^{{\gamma _p}}}}}{{\sum\limits_{i = 1}^{{w_p}} {{c_{p,i}}} }},
\end{equation}
where \(T_f^{(a)}(B)\) is the time for forward pass of the $P_a$ on a batch of size \(B\), \(T_f^{(p)}(B)\) is the time for forward pass of the $P_p$ on a batch of size \(B\), \(\gamma_a\), \(\lambda_a\), \(\gamma_p\), and \(\lambda_p\) are the proportionality constants. For simplicity, if all \(w_p\) workers are assigned equally, it might become \(T_f^{(a)}(B) = \frac{{{\lambda _a}{B^{{\gamma _a}}}{w_a}}}{{{C_a}}}\) and \(T_f^{(p)}(B) = \frac{{{\lambda _p}{B^{{\gamma _p}}}{w_p}}}{{{C_p}}}\). Similarly, let \(\beta_a\) and \(\beta_p\) be the constant for the backward pass. Thus, we have: 
\begin{equation}\label{eq-8}
T_b^{(a)}(B) = \frac{{{\varphi _a}{B^{{\beta _a}}}{w_a}}}{{{C_a}}},T_b^{(p)}(B) = \frac{{{\varphi _p}{B^{{\beta _p}}}{w_p}}}{{{C_p}}}.
\end{equation}
We give the forward and backward propagation time of the top model part of $P_a$ as follows:
\begin{equation}\label{eq-9}
T_{top}^{(a)}(B) = \frac{{\lambda _a^{'}{B^{\gamma _a^{'}}}{w_a}}}{{{C_a}}} + \frac{{\varphi _a^{'}{B^{\beta _a^{'}}}{w_a}}}{{{C_a}}}.
\end{equation}
Next, we consider the communication delay within the system pipeline. Let \( E \) denote the size of the embedding sent by the $P_p$ and \( G \) the size of the gradient sent by the $P_a$. Each iteration involves two primary communications: $P_p$ sends the embedding to $P_a$, and $P_a$ sends the gradient back to $P_p$. Therefore, the total communication delay for each iteration can be expressed as:
\begin{equation}
    {T_{emb}} = \frac{E}{{{B_b}}},{T_{grad}} = \frac{G}{{{B_b}}}.
\end{equation}
where \( B_b \) denotes the bandwidth capacities of the system. Since the semi-asynchronous aggregation within the PS is performed internally within each participant, the communication delays from this step can be ignored, as they are generally fixed constants. %Therefore, when evaluating the system communication delay, we focus solely on the delays caused by inter-party communication.

\para{Remark on Pipelining/Asynchronous Pub/Sub.} With a Pub/Sub architecture, one can sometimes overlap the next batch’s forward pass at the $P_p$ with the $P_a$’s backward pass from the previous batch. In a fully pipelined system with enough buffering, the overall iteration time can be lower than the naive sum above. Nonetheless, many system analyses still approximate iteration time by a ``critical path'' sum or a maximum of partial sums~\cite{ye2024asteroid,zheng2022alpa}. For simplicity, we continue with the additive formula here, but in practice, pipelining would reduce that total somewhat. %Hence, a simplistic upper bound on per‐iteration time would be:
%\begin{equation}\label{eq-11}
%\begin{aligned}
%T_{\text{iter}} &= T_f^{(p)} + T_{\text{emb}} + T_f^{(a)} + T_b^{(a)} + T_{\text{grad}} \\
%                &= \frac{\gamma B}{\sum\limits_{j=1}^{w_p} c_{p,j}} + \frac{E}{B_b} + \frac{\alpha B}{\sum\limits_{i=1}^{w_a} c_{a,i}} + \frac{\beta B}{\sum\limits_{i=1}^{w_a} c_{a,i}} + \frac{G}{B_b}.
%\end{aligned}
%\end{equation}
\subsection{System Planning Phase}\label{4-4}
\para{Optimization Problem Formulation.} Considering privacy concerns and network access restrictions, it is challenging for participants to collaboratively perform fine-grained pipeline operations. To address this, our approach is to estimate the computation and communication time in the Pub/Sub scenario based on the time observed in a synchronous scenario, as shown in Fig. \ref{fig-2}. This estimation allows us to construct an optimization model to determine the optimal hyperparameters, i.e., the number of workers and batch size, for initialization. By leveraging this model, we aim to balance computation and communication costs while ensuring efficient system performance under the constraints of privacy and limited network collaboration. According to Eq. \eqref{eq-4}, we can rewrite the formal expression of $T_A$ and $T_P$ as:
\begin{equation}
{T_A} = T_f^{(a)} + T_b^{(a)} + T_{top}^{(a)} + {T_{grad}},{T_P} = T_f^{(p)} + T_b^{(p)} + {T_{emb}}.  
\end{equation}
Then, we rewrite Eq. \eqref{eq-4} as follows:
\begin{equation}\label{eq-13}
\min \max (T_f^{(a)} + T_b^{(a)} + T_{top}^{(a)} + {T_{grad}},T_f^{(p)} + T_b^{(p)} + {T_{emb}}).
\end{equation}
In Eq. \eqref{eq-13}, we want to choose the optimal hyperparameters, i.e., \(w_a \in \{P, P+1, \ldots, Q\}\) , \(w_p \in \{M, M+1, \ldots, N\}\), an integral (or real) batch size $1 \le B \le {B_{max}}$ (bounded above by some feasible maximum, i.e., memory constraints), to optimize the goal. We assume that each party has its own memory constraint per worker. Thus, we follow \cite{ye2024asteroid} to specify the memory usage functions as
\begin{equation}
{M_A}(B) = {M_{A0}} + {\rho _A}{B^\chi },{M_P}(B){\rm{ }} = {M_{P0}} + {\rho _P}{B^\chi },
\end{equation}
where \(M_{A0}\) and \(M_{P0}\) are the base memory consumptions at the active and passive parties respectively, and  \(\rho _A,\rho _P\) (with exponent \(\chi\)) capture the extra memory needed per worker as a function of the minibatch size \(B\). If the maximum available memory per worker at the $P_a$ is \(\bar{M}_A\) and at the $P_p$ is \(\bar{M}_P\), then the memory constraints become $B \le {\left( {\frac{{{{\bar M}_A} - {M_{A0}}}}{{{\gamma _A}}}} \right)^{1/\chi }},B \le {\left( {\frac{{{{\bar M}_P} - {M_{P0}}}}{{{\gamma _P}}}} \right)^{1/\chi }}.$ Thus, we define the overall feasible maximum batch size due to memory as
\begin{equation}
{B_{\max }} = \min \left\{ {{{\left( {\frac{{{{\bar M}_A} - {M_{A0}}}}{{{\rho _A}}}} \right)}^{1/\chi }},{\mkern 1mu} {{\left( {\frac{{{{\bar M}_P} - {M_{P0}}}}{{{\rho _P}}}} \right)}^{1/\chi }}} \right\}.
\end{equation}
We assume that the candidate minibatch sizes are taken from a discrete set, i.e., $\mathcal{B}=\{B_1,B_2,\dots,B_R\},$ but only those values that satisfy \(B\le B_{\max}\) are feasible. Since both parties must finish their computations before proceeding to the next iteration, the overall per-iteration delay is the maximum of the two computation delays plus the communication delay:
\begin{equation}
\tiny
\begin{aligned}
\min \mathcal{O} ({w_A},{w_P},B) = \mathop {\min }\limits_{_{{w_a},{w_p},B \le {B_{\max }}}} \left\{ {\max \left( {T_f^{(a)} + T_b^{(a)} + T_{top}^{(a)},T_f^{(p)} + T_b^{(p)}} \right) + \frac{{E + G}}{{{B_b}}}} \right\}.  
\end{aligned}
\end{equation}

\para{Dynamic Programming Algorithm Design.} Because the decision space (over \(w_a\), \(w_p\), and \(B\)) is discrete, we now describe a dynamic programming approach to search for the optimal configuration. We define a dynamic programming state by the triplet \((i,j,r)\), where, \(i\) indexes the candidate active worker count: \(w_a=M+i-1\) for \(i=1,2,\dots,(N-M+1)\), \(j\) indexes the candidate passive worker count: \(w_p=P+j-1\) for \(j=1,2,\dots,(Q-P+1)\), and \(r\) indexes the candidate minibatch size: \(B=B_r\) for \(r=1,2,\dots,R\), with the additional constraint \(B_r\le B_{\max}\). The cost associated with state \((i,j,r)\) is defined as
\begin{align}
\tiny
    {\rm{Cost}}(i,j,r) = \max \Bigg\{ &
    \frac{
        (\lambda_a B_r^{\gamma_a} + \lambda_a' B_r^{\gamma_a'} + \varphi_a B_r^{\beta_a} + \varphi_a' B_r^{\beta_a'})(M + i - 1)
    }{C_a},  \notag \\
    & \frac{
        (\lambda_p B_r^{\gamma_p} + \varphi_a B_r^{\beta_p})(P + j - 1)
    }{C_p} \Bigg\}.
\end{align}
The objective is to find the state \((i^*,j^*,r^*)\) that minimizes this cost. The above dynamic programming solution (Algo. \ref{alg:dp_config}) and the pseudo code of \texttt{PubSub-VFL} (Algo. \ref{alg:pubsub_vfl}) can be found in the Appendix \ref{algo}.








==> sections/relatedwork.tex <==
\section{Related Work}
\para{Split Learning-based Vertical Federated Learning.} Split Learning (SL)~\cite{abuadbba2020can,thapa2022splitfed} has emerged as a promising technique for VFL in scenarios where data is vertically partitioned across organizations. In SL-based VFL, participants collaboratively train a model by splitting the training process across multiple entities, ensuring that raw data never leaves local environments. For instance, \citet{poirot2019split} proposed a SL-based VFL approach for healthcare applications, demonstrating its ability to preserve data privacy while achieving high model performance. %Similarly, \citet{zhao2024vertimrf} investigated SL-based VFL with Differential Privacy (DP), further reducing the risks of data leakage. 
However, these approaches often face challenges related to low computational resource utilization and synchronization issues, especially in heterogeneous environments. These limitations highlight the need for alternative architectures to address the scalability and efficiency challenges inherent in SL-based VFL systems.

\para{Vertical Federated Learning with PS.} The integration of PS~\cite{li2014scaling} architectures into (V)FL systems has garnered attention due to its potential to improve scalability and flexibility. Early efforts such as \cite{bonawitz2019towards} explored using PS architecture to achieve efficient aggregation and distribution of model parameters, simplifying the coordination of multiple participants, but these were primarily focused on horizontal FL settings. More recently, \cite{wu2023falcon,FATE2023,PaddleFL2023} demonstrated the applicability of PS architectures in VFL contexts, showing improvements in resource utilization and dynamic participant management. \citet{castiglia2023flexible} extended this approach by introducing hierarchical PS architectures, allowing for better load balancing and reduced latency in VFL. However, these solutions still grapple with issues such as decoupling from the unique step in VFL (i.e., ID alignment) to further unlock the potential of PS. %This rigidity has spurred interest in hybrid architectures, such as Pub/Sub systems, which offer greater flexibility and adaptability by decoupling embedding producers and consumers.

\para{Asynchronous Vertical Federated Learning.}
Asynchronous training~\cite{zhang2024asynchronous,chen2020vafl,zhang2021secure} methods have gained traction in VFL to address the inefficiencies caused by straggler effects and the need for strict synchronization. Asynchronous VFL (AVFL) enables participants to train and exchange intermediate results independently, significantly improving system throughput and scalability. Recent works, such as those by \citet{zhang2021secure}, have demonstrated the efficacy of AVFL in mitigating delays caused by slow participants, thereby enhancing the overall efficiency of the learning process. Nevertheless, asynchronous methods introduce new complexities, including staleness in gradients and potential divergence of models. To tackle these issues, recent research has focused on developing consistency models~\cite{liu2021adaptive,koloskova2022sharper} and adaptive asynchronous strategies \cite{zhang2023timelyfl}. We summarize the comparison between existing methods and PubSub-VFL in Table \ref{tab:vfl_comparison} in Appendix.
